Learning Non-robustness using Simulation-based Testing: a Network Traffic-shaping Case Study

An input to a system reveals a non-robust behaviour when, by making a small change in the input, the output of the system changes from acceptable (passing) to unacceptable (failing) or vice versa. Identifying inputs that lead to non-robust behaviours is important for many types of systems, e.g., cyber-physical and network systems, whose inputs are prone to perturbations. In this paper, we propose an approach that combines simulation-based testing with regression tree models to generate value ranges for inputs in response to which a system is likely to exhibit non-robust behaviours. We apply our approach to a network traffic-shaping system (NTSS) -- a novel case study from the network domain. In this case study, developed and conducted in collaboration with a network solutions provider, RabbitRun Technologies, input ranges that lead to non-robustness are of interest as a way to identify and mitigate network quality-of-service issues. We demonstrate that our approach accurately characterizes non-robust test inputs of NTSS by achieving a precision of 84% and a recall of 100%, significantly outperforming a standard baseline. In addition, we show that there is no statistically significant difference between the results obtained from our simulated testbed and a hardware testbed with identical configurations. Finally we describe lessons learned from our industrial collaboration, offering insights about how simulation helps discover unknown and undocumented behaviours as well as a new perspective on using non-robustness as a measure for system re-configuration.

==> algorithm.tex <==
\section{algorithm}

\begin{algorithm}[]
\caption*{Subroutines of Boundary Test}
    \begin{algorithmic}[1]
        \Procedure{GeneratePoints}{Ranges}
            \State point $\gets$ [0 ,..., 0] \Comment an array of size n that will be the new point
            \For{$ i \gets 0 \to n$}
                \State point[i] $\gets$ Randomly generate a number based on Ranges[i]
            \EndFor
            \State \textbf{return} point
        \EndProcedure 
        \\
        \Procedure{SimulateData}{member}
            \Comment Simulates the given member of the population
            \State Generate nuttcp traffics based on member
            \State ProbeOutput $\gets$ Read outputs of probe
            \State \textbf{return} ProbeOutput
        \EndProcedure
        \\
        \Procedure{LabelData}{Pop, Labels}
            \Comment Labels the probe outputs
            \For{each probe column in Pop}
                \State Update the value of the column based on the given Labels
            \EndFor
            \State \textbf{return}
        \EndProcedure
        \\
        \Procedure{FindBoundaryRules}{Trees}
            \State BoundaryRules $\gets$ []
            \For{each tree in Trees}
                \State rule $\gets$ Find the point where the label of the leaves changes from Good to Bad or Bad to Good
                \State Get the paths (root to leaf) and add them to the BoundaryRules
            \EndFor
            \State \textbf{return} BoundaryRules
        \EndProcedure 
        \\
        \Procedure{ExtractRanges}{X, BoundaryRules, Ranges}
            \State NewRanges $\gets$ Ranges
            \For{$ i \gets 0 \to len(BoundaryRules)$}
                \For{$ j \gets 0 \to len(X)$}
                    \If{ BoundaryRules[i] contains variable X[j]}
                        \State Update the ranges of X[j] in NewRanges
                    \EndIf
                \EndFor
            \EndFor
            \State \textbf{return} NewRanges
        \EndProcedure
        \\
        \Procedure{Should I write the procedure of Adaptive Random Search?}{}
        \EndProcedure
        \algstore{myalg}
    \end{algorithmic}

\end{algorithm}

\begin{algorithm}[]
\caption{Boundary Tests}
    \begin{flushleft}
    \hspace*{\algorithmicindent}\textbf{Input:} \\
    \hspace*{\algorithmicindent} -X: Name of the input variables (TINs) \\
    \hspace*{\algorithmicindent} -Labels: A set of Labels for discretization \\
    \hspace*{\algorithmicindent} -Ranges: The default ranges of X \\
    \hspace*{\algorithmicindent}\textbf{Output:} n decision trees and pairs of boundary rules \\
    \end{flushleft}
    \begin{algorithmic}[1]    
        %\algrestore{myalg}
        \Procedure{Boundary Tests}{}
            \State Pop $\gets$ []
            \For{$ i \gets 0 \to 100$}
            \Comment Generates 100 initial points based on the default ranges
            \State newpoint $\gets$ 
            \Call{GeneratePoints}{Ranges}
            \State ProbeOutput $\gets$ 
            \Call{SimulateData}{newpoint}
            \State Append newpoint and ProbeOutput to Pop
            \EndFor
            
            
            \Repeat
            
                \Call{LabelData}{Pop, Labels} \Comment Discretizes the desired probe output columns based on the given Labels 
                \State Build n Decision Trees based on Pop
                \State BoundaryRules $\gets$ 
                \Call{FindBoundaryRules}{Trees} \Comment Gets the boundary rules of each tree
                \State NewRanges $\gets$
                \Call{ExtractRanges}{X, BoundaryRules, Ranges} \Comment Gets the new ranges of each input variable based on the boundary rules
                \State NewPop $\gets$ Use adaptive random search to generate new points based on the new ranges
                \For{each member in NewPop} 
                    \State ProbeOutput $\gets$ 
                    \Call{SimulateData}{member}
                    \State Append member and ProbeOutput to Pop
                \EndFor
                    
                    
            \Until{time has run out}
            \State \textbf{return} Trees and BoundaryRules
        \EndProcedure

    \end{algorithmic}

\end{algorithm}


Explain the algorithms. 


NEEDS a good running example. 

==> background.tex <==
\section{Background Concepts}
\label{sec:background}
\subsection{Network Protocols}
\textbf{TCP:}
Transmission Control Protocol (TCP) is a transport layer communication standard that allows computing devices to communicate over a network. TCP is connection oriented; meaning that it guarantees that data and messages are delivered successfully through networks. Common applications of TCP include peer-to-peer sharing methods such as File Transfer Protocol (FTP) and sending and receiving emails through Internet Message Access Protocol (IMAP) \cite{TCP}. 
\\
\textbf{UDP:}
User Datagram Protocol (UDP) is a message-oriented (connectionless) transport layer communication standard that delivers packets immediately to the destination without first establishing a connection. UDP is mainly used for time-sensitive applications such as videos and games.
\\
\textbf{ICMP:}
Internet Control Message Protocol (ICMP) is a connectionless network layer protocol and is mainly used by routers to diagnose communication problems in networks. 

In the terms of the network diagnosing, TCP can be used to test the scenarios where TCP segments are lost or delayed. UDP is used to test the quality of latency-sensitive applications such as VOIP, livestreams, video calls over the network. Finally, ICMP pings are simply used for network reachability and route tracing. 


User generated traffic is not ICMP. It is either TCP or UDP. For synthetic/test, when TCP? and when UDP?

%\subsection{Differentiated Services}
%Differentiated services or diffserv is a network quality of service mechanism. The basic idea of diffserv is to classify network packets under different classes. Specifically,  the information in the packet IP headers are used to classify packets. In particular, packet IP headers include an 8-bit Differentiated Services (DS) and 6 most significant bits of this field is referred to as \emph{differentiated services Code Point (DSCP)}. There are five main classes of DSCP:
%\begin{enumerate}
%    \item \textbf{Lower-Effort (LE):} is referred to a low urgency traffic where packets of higher precedence can take over it in a congested network.
    
%    \item \textbf{Default Forwarding (DF):} also called Best-Effort refers to any traffic that does not fit into other mentioned classes.
    
%    \item \textbf{Assured Forwarding (AF):} It allows the operator to guarantee delivery of the packet. 
    
%    \item \textbf{Expedited Forwarding (EF):} is related to low-loss, low-latency traffic and must be given highest priority.
    
%    \item \textbf{Class Selector (CS):} Diffserv specifies this class to ensure backward compatibility with network devices that still utilise the precedence field (a field that was used in TOS bytes to mark priority traffic).
%\end{enumerate}


%The value of DSCP for each packet depends on the dscp class of the packet. For example, multimedia streaming applications (Assured Forwarding class) may have dscp value of 011010 whereas dscp value of low-priority data (CS1) can be 001000.

%TABLE TO SHOW THE RANGE OF THE VALUES OF DSCP CLASSES.

%Diffserv techniques are parameterized by a mapping that relate the packet DSCP values to the priority classes. 
%Diffserv classes can themselves be routed into different priority classes (or tins) based on a mapping. On a network setting, there can be n classes and each class is serviced based on a WRR algorithm \cite{CAKE}. 



==> constraintGen.tex <==
\section{Constraints or Invariants Generation}

Suggested Constraints (based on Pat's mapping): 
\begin{itemize}
    
    \item The bandwidth threshold of a high priority class is more than the bandwidth threshold of a low priority class. \\
    $ \forall c_i , c_j \ \mathit{prio}(c_i) \geq \mathit{prio}(c_j) \rightarrow \mathit{bw$-$th}(c_i) \geq \mathit{bw$-$th}(c_j)$
    
    \item When we have two traffics running parallelly and entering different tins, the actual bandwidth of the traffic entering a low priority tin will be very close to the bandwidth threshold of that tin. As a result, the actual bandwidth of the tin entering the higher priority tin will be the remaining available bandwidth. \\
    $ \forall tr_i , tr_j \ M(tr.dscp(i)) < M(tr.dscp(j)) \ \vee \ \mathit{prio}(M(tr.dscp(i))) > \mathit{prio}(M(tr.dscp(j))) \ \rightarrow tr.\mathit{actual$-$bw}(j) = \mathit{bw$-$th}(M(tr.dscp(j)) \ \pm \epsilon \ \land \ tr.\mathit{actual$-$bw}(i) = \mathit{total$-$bw}(sc) - tr.\mathit{actual$-$bw}(j) $
    
    \item The total bandwidth will be equally splitted between the two traffics that enter the same tin at the same time. \\
    $ \forall tr_i , tr_j \ M(tr.dscp(i)) = M(tr.dscp(j)) \rightarrow tr.\mathit{actual$-$bw}(i) = tr.\mathit{actual$-$bw}(j) $
    
    \item Latency 
    
    
\end{itemize}


==> oldstuff.tex <==
%Environment inputs characterize the incoming traffic to the system. There are three main categories of traffic in this project: Baseline, Random, Ping. This includes the DSCP value, duration of sending packets, the packet bandwidth, source and destination IPs and the protocol type (TCP, UDP and ICMP). These inputs determine what types of traffic are generated in a SoHo system by their users (e.g., playing games, zoom calls, netflix and internet browsing). These traffics run in a sequential order (with the same duration) during a scenario. Figure 1 depicts the domain model of our SoHo system and the range of the parameters.

%\begin{equation}
%    bt.trafficsequence \rightarrow asOrderedSet()
%\end{equation}
%\begin{equation*}
%    rt.trafficsequence \rightarrow asOrderedSet()
%\end{equation*}
%\begin{equation*}
%    pt.trafficsequence \rightarrow asOrderedSet()
%\end{equation*}

%\begin{equation}
%    bt.duration = rt.duration = pt.duration
%\end{equation}

%The parameters of the Baseline traffic sequences are constant and will not change during a simulation scenario. The second category of traffic is Random where the parameters are dynamic and can be changed during a scenario. Finally, Ping traffic is related to the traffic generated for determining the latency, jitter and loss of the destination IPs. Baseline and Random traffics are generated using a traffic generation tool called nuttcp \cite{nuttcp} and Ping traffics are generated by dpinger \cite{dpinger} and hping3 \cite{hping3}.
 
%System parameters include diffserv mapping and total requested bandwidth threshold for the router.


%The router on the network is configured to differentiate and classify traffic based on this mapping. Specifically, all the sequences of Baseline ($bt$), Random ($rt$), and Ping traffics ($pt$) are routed to specific tins based on their DSCP values: 
%\begin{equation}
%    \begin{multlined}
%        bt \rightarrow forall (bt1 : Baseline Traffic | MA.index(bt1.dscp) = bt1.tin) 
%    \end{multlined}
%\end{equation}
%\begin{equation*}
%    rt \rightarrow forall (rt1 : Random Traffic | MA.index(rt1.dscp) = rt1.tin)
%\end{equation*}
%\begin{equation*}
%    pt \rightarrow forall (pt1 : Ping Traffic | MA.index(pt1.dscp) = pt1.tin)
%\end{equation*}

%In our setting, the Baseline traffic will be routed to one tin and each tin will have k Random traffics and one Ping traffic. As a result, the summation of number of traffics entering the tins should be equal to the total number of available traffic:    
%\begin{equation}
%    \displaystyle \sum^7_{i=0} k_i + \sum^7_{i=0} p_i + 1 = n + 8 + 1
%\end{equation}
%where $k_i$ is the number of random traffics and $p_i$ is the number of ping traffics entering tin i.

%OCL:
%\begin{equation*}
%can we express it in this way?:
%    \begin{multlined}
%       tin \rightarrow collect(tin.rt %\rightarrow size() + tin.bt \rightarrow %size() \\ + tin.pt \rightarrow size()) %\rightarrow sum() = n + 9
%    \end{multlined}
%\end{equation*}
%\begin{equation}
%    \begin{multlined}
%      tin \rightarrow forall (tin1: Tin | tin1.rt \rightarrow size() \leq n \ and \\ tin1.bt \rightarrow size() \leq 1 \ and \ tin1.pt \rightarrow size() = 1) 
%    \end{multlined}
%\end{equation}
%Moreover, each tin has a fixed bandwidth threshold which is a portion of total requested bandwidth. The bandwidths of traffics entering the tins will not exceed this threshold:
%\begin{equation}
%   \begin{multlined}
%   t \rightarrow forall (t1: Traffic | t1.tin.bandwidththreshold \geq \\ t1.allocatedbandwidth )
%\end{multlined} 
%\end{equation}
%Where $Traffic$ is either Random or Baseline traffic and $t$ is a collection of it.
%In a simulation scenario, there will be one Baseline traffic, a number of Random traffics and 8 ping traffics. All traffics will run parallelly (at the same time) and each traffic will be divided into a sequence of small traffics where DSCP value, start time, end time and duration can be specified. 


%The output of the system is retrieved by dpinger and hping 3 which are tools for monitoring latency and loss on a network connection \cite{dpinger} \cite{hping3}. In fact, the Ping traffics will help the dpinger and hping3 to determine latency, jitter, loss and MOS. Moreover, the allocated bandwidths to traffic tr is obtained from nuttcp reports. The allocated bandwidth indicates what chunk of the total requested bandwidth was dedicated to a specific traffic with respect to the bandwidth threshold of the tin.
%\begin{equation}
%    \begin{multlined}
%         \displaystyle \sum^n_{i=1} rt_i.allocatedbandwidth + bt.allocatedbandwidth \\ = totalrequestedbandwidth 
%    \end{multlined}
%\end{equation}
%OCL:
%\begin{equation*}
%    \begin{multlined}
%       rt.allocatedbandwidth \rightarrow sum() + bt.allocatedbandwidth \\ = totalrequestedbandwidth
%    \end{multlined}
%\end{equation*}


%A large number of metrics are produced as the result of monitoring the system outputs. It is often not possible to convert all these values into a single number.  


\section{Ideas}

For each class $c_j$, we say the service is good if the MOS factor is 4.41, the latency is less than 5000 and the percentage allocated BW is close 100\%. 

 

We pose a number of research questions: 

\textbf{RQ1. (Random Data Generation)} \emph{Is there a strict ordering on the service of the different classes?}


To answer this question, we generate input traffic data using a simple random search. We then use the data to learn such predicates:  

$\forall i, j, F_i < F_j \implies c_i < c_j$

where $F$ can be replaced by latency, MOS, jitter, or percentage BW. 

We say TIN $i$ is better than TIN $j$, if $i$ has higher percentage BW than $j$, and if $i$ has lower latency than $j$, and if $i$ has higher MOS than $j$. 

It seams that we are able to learn the above predicates over the data we generate with high degree of confidence. So the class (TIN) 8 is the best and (TIN) 0 is the worst. But We have to see if there is a clear ordering between TIN 8 and TIN 7 as well?

\textbf{First-TODO.} Learning predicates to determine strict ordering over TINs. We probably do not learn any ordering between 8 and 7 or between 0 and 1, but there will some other pairwise predicates we learn over the TINs. 


\textbf{RQ2. (Stress Testing)} \emph{Is it possible to find input traffics that make some high priority TINs perform poorly?}




To answer this, we run search algorithms that aim to make the better TINs perform worse. We run a Hill Climbing search with a fitness that penalizes the degradation of latency on higher TINs more.

$Fitness = \sum i* latency-level$

Our goal is to see if we can push the higher TINs to generate low service. We also try to learn more predicates to describe the behaviour of these TINs: 


$\forall i, TIN_i-reqBW > TIN_i-Threshold => TIN_i-Latency > 5000$

Also, is there a cap (upper bound) on latency for higher TINs?

$TIN_8-latency < 6000$
$TIN_8-BWpercentage > 0.99$

While there is a lower bound for lower TINs?

\textbf{Second-TODO.} Are we able to learn predicates that specify upper bounds for higher priority TINs for their latency/jitter and lower bound for their percentageBW? Are we able to learn predicates that specify lower bounds for lower priority TINS for their latency/jitter and upper bound for their percentageBW? Are we able to learn predicates that for higher priority TINs that provide a lower bound on latency when their input BW goes higher than their threshold BW? Are we able to learn predicates for lower priority TINs that provide a higher bound on latency when their input BW is lower than their threshold BW?


Any other predicates showing the relationship between input and output?

The above predicates show that some TINs always doing significantly more poorly than others. On the hand, we cannot put all the traffic on the higher TINs since the last predicates show that higher priority TINs also degrade when we put too much traffic on them.

On more open issue here: What inputs impacts the total MOS? Or in other words total MOS is correlated with which input? This will help us learn metamorphic rules. 


\textbf{RQ3. (Regression Learning)} \emph{What distribution of input traffics (requested BWs) lead to good service on all classes?}

We build logistic regression models to help build these distributions. 



\begin{algorithm}[]
\caption*{Subroutines of PTOG}
    \begin{algorithmic}[1]
        
        \Procedure{BuildInitialTrees}{Population}
            \Comment Builds initial trees from initial population
            \State InitialProbeOutput $\gets$ \Call{SimulateData}{Population}
            \State InitialLabeledOutput $\gets$ \Call{LabelData}{InitialProbeOutput}
            \State Build n decision trees ${Tree_1 , ... , Tree_n}$ based on Population and InitialLabeledOutput and store them in Trees
            \State \textbf{return} Trees
        \EndProcedure
        \\
        \Procedure{GenerateDataFromPath}{Region}
            \Comment Build a small population from the Region
            \State Pop = []
            \While{$len(Pop) < 10$}
                \State Use adaptive random search to find a new member and add it to the Pop
            \EndWhile
            \State \textbf{return} Pop
        \EndProcedure
        \\
        \Procedure{SimulateData}{Population}
            \Comment Simulates the members of the population and returns their probe readings
            \State ProbeOutput = []
            \For{$i \gets 0 \to len(Population)$}
                \State Generate nuttcp traffics based on Population[i]
                \State $Output \gets$ Read outputs of probe
                \State Add $Output$ to ProbeOutput
            \EndFor
            \State \textbf{return} ProbeOutput
        \EndProcedure
        \\
        \Procedure{LabelData}{ProbeOutput}
            \Comment Labels the probe outputs
            \State LabeledOutput $\gets$ Label values of ProbeOutput based on Labels
            \State \textbf{return} LabeledOutput
        \EndProcedure
        \algstore{myalg}
    \end{algorithmic}

\end{algorithm}

\begin{algorithm}[]
\caption{Partial Test Oracle Generation(PTOG)}
    \begin{flushleft}
    \hspace*{\algorithmicindent}\textbf{Input:} \\
    \hspace*{\algorithmicindent} -Labels: A set of Labels to discretize data \\
    \hspace*{\algorithmicindent} -flag: Critical or Diversity \\
    \hspace*{\algorithmicindent}\textbf{Output:} n decision trees \\
    \end{flushleft}
    \begin{algorithmic}[1]    
        %\algrestore{myalg}
        \Procedure{Partial Test Oracle Generation}{}
            \State Select an initial input population set $Population$ randomly
            \State Trees $\gets$ \Call{BuildInitialTrees}{Population}
            
            \Repeat
                \For{$i \gets 1 \to n$}
                    \If {flag is Critical}
                        \State Region $\gets$ Randomly choose a critical path from Trees[i]
                    \ElsIf {flag is Diversity}
                        \State Region $\gets$ Randomly choose a path from Trees[i]
                    \EndIf
                    \State $NewPop \gets $ \Call{GenerateDataFromPath}{$Region$}
                    \State $NewProbeOutput \gets $ \Call{SimulateData}{$NewPop$}
                    \State $NewLabeledOutput \gets $ \Call{LabelData}{$NewProbeOutput$}
                    \State $Population \gets Population \cup NewPop $
                    \State Rebuild decision trees ${Tree_1, ... , Tree_n}$ based on $Population$ and $NewLabeledOutput$ and store them in Trees
                \EndFor    
            \Until{time has run out}
            \State \textbf{return} Trees
        \EndProcedure

    \end{algorithmic}

\end{algorithm}


$ \mathit{effective latency} = \mathit{latency} + \mathit{jitter} \times \mathit{latency impact} + \mathit{compTime} $


\emph{compTime} is a constant value for computation time. In our calculation, we have chosen \emph{latencyimpact} and \emph{compTime} values equal to 2 and 10 respectively. Second, we use \emph{effectivelatency} to define R-factor which is also a metric to measure quality of audio:

    $ \mathit{R\text{-}factor} = \begin{cases}
    \mathit{defaultR} - \frac{\mathit{effectivelatency}}{40}, \ \ \          \mathit{effectivelatency} < 160\\
    \mathit{defaultR} - (\frac{\mathit{effectivelatency} - 120}{40}),\ \ \   o.w
    \end{cases}$

where \emph{defaultR} is by default 93 but can be changed depending on the value of \emph{effectivelatency}. For high values of \emph{effectivelatency} we assign a small \emph{defaultR} value. For example, if \emph{effectivelatency} is more than 500, \emph{defaultR} becomes 10. Next, we revise \emph{R-factor} to add the effect of loss:
$ \mathit{R\text{-}factor} = \mathit{R\text{-}factor} - (\mathit{loss} \times 2.5) $
\\


For each simulation scenario $\mathit{sc}$, we request a total bandwidth denoted by $\mathit{total$-$bw}(sc)$. The total bandwidth is a nominal value that we set as input for our simulations to be executed on a given platform. The thresholds of the classes are a proportion of a total requested bandwidth. Specifically, the higher priority classes are allocated less proportions (e.g. 25\%) than lower priority classes (e.g. 90-100\%) \cite{CAKE}. The idea is that there is a key tradeoff between priority and bandwidth; meaning that more latency-sensitive traffic requires less bandwidth \cite{CakeTechnical}. For example, if we have a traffic shaping system with three classes and requested bandwidth of 100 Mbit, the thresholds of the highest and lowest classes are 25 Mbit and 100 Mbit respectively. 
The total requested bandwidth for a simulation is typically set to be close (10\% more) to the capacity of the simulation platform on which the scenario is executed (see Section~\ref{simplat}). For example, for the virtual environment the total requested bandwidth is 1820 Mbit. 



%\begin{figure}[]
%    \centering
%    \includegraphics[width=\columnwidth]{figs/inputoutputexample.PNG}
%    \caption{Examples of system input and output}\label{fig:inputoutputexample}
%\end{figure}


%Latency (also called round trip time) is referred to the time it takes for a packet to travel from a source to the destination and back. A low latency network connection typically has minor delay times and indicates a network with a higher quality of service. Jitter is the standard deviation of latency and indicates the variability of latency over time. Packet loss is referred to the number of packets that fail to reach their intended destination. Packet loss can affect any application, but the quality of applications that need real-time packet delivery (e.g. video, audio and games) are the most affected when there is packet loss~\cite{loss}.


%As discussed in Section~\ref{sec:background}, traffic shaping mechanisms are parameterized by a mapping that relate DSCP codes of network packets to the diffserv classes.  We denote the diffserv mapping by a function $M:\{0,\ldots, 63\} \rightarrow \{1, \ldots, n\}$ that maps the 64 DSCP values to a diffserv class between $1$ to $n$. For example, $M(0) = 2 $  assigns any packet with DSCP value $0$ to $c_2$ among our diffserv priority classes. A diffserv mapping is a pre-requisite to a differentiated service mechanism and has a great impact on the desirable functioning of the system. Our goal in this paper is use explainable models to provide guidelines to help specify such mapping so that the system behaves as desired. 





%Each simulation scenario $\mathit{sc}$ is executed over a simulation duration $[0..T]$ divided into equal simulation steps $\delta$. In other words, each simulation scenario is executed for $k$ steps where $k = \frac{T}{\delta}$. Each simulation scenario $\mathit{sc}$ is executed on a simulation platform which can be fully virtual, hybrid or the real system (see Section~\ref{simplat}).


%Similarly, on the hybrid platform, we set the total bandwidth of ?? for our simulations.  




%Each simulation scenario $\mathit{sc}$  involves generating and running a number of (independent) traffic streams in parallel. Each traffic $\mathit{tr}$ is generated to transmit data from a source $\mathit{tr.src}$  to a destination $\mathit{tr.dst}$ and follows one of the following protocols: TCP, UDP and ICMP. In addition, each traffic $\mathit{tr}$ has a duration $\mathit{tr.duration}$, a start time $\mathit{tr.start}$, and an end time $\mathit{tr.end}$. Each traffic may run for the whole or only part of the simulation duration $T$. The start and the end times of each traffic are within the simulation duration. That is, for each traffic $\mathit{tr}$, we have $\mathit{tr.duration} = \mathit{tr.end} - \mathit{tr.start}$. In addition, $\mathit{tr.duration} \leq T$ for every traffic $\mathit{tr}$. 


%For each traffic $\mathit{tr}$, we need to set a requested bandwidth that we denote by $\mathit{tr.req$-$bw}$. There is no specific constraint on the requested bandwidth for an individual traffic, but, as we will discuss later, the actual bandwidth that will be allocated to the traffic by the traffic shaping mechanism may not reach the requested bandwidth value. 


%Traffics are generated for two different purposes: test (synthetic) or probe. We use an attribute \emph{trafficType} in Figure~\ref{fig:domainmodel} to differentiate these two different usages of traffics, and we refer to the traffic type by $\mathit{tr.type}$.  Both types of traffics execute over the simulation time steps $1$ to $k$ where $k = \frac{T}{\delta}$. For the traffic generated for testing purposes, we may choose to modify the DSCP of test traffic during the simulation time steps or keep the DSCP fixed over the entire duration of the test traffic. The latter case represent ?? and the former represent ??. 


%As discussed earlier, the traffic dscp value determines the class to which the traffic is redirected by the traffic shaping mechanism. We refer to the dscp value of a traffic $\mathit{tr}$ at step $i$ by $\mathit{tr.dscp(i)}$. The diffserv class of traffic $\mathit{tr}$ at step $i$ is then determined by $M(\mathit{tr.dscp(i)})$ where $M$ is the diffserv mapping function defined earlier. We refer to a  traffic$\mathit{tr}$ whose dscp remains unchanged during the simulaiton (i.e., $\mathit{tr.dscp(1)} = \mathit{tr.dscp(2)}=  \ldots =  \mathit{tr.dscp(k)}$ where $k$ is the number of simualtion step) as a \emph{baseline} or \emph{bulk} traffic. 

%\begin{figure}[]
%    \centering
%    \includegraphics[width=\columnwidth]{figs/domain model 7.png}
%    \caption{Domain model of SOHO system}\label{fig:domainmodel}
%\end{figure}


 %The purpose of probe traffic is to measure the latency and loss values for each class of our traffic shaping system. 
 %\textbf{sh:  EXPLAIN how a traffic monitor tool works}.
 %In our work, we create two types of probe traffics for each diffserv class $c$ and those probe traffics do not change their diffserv classes during the simulation. The first type of probe traffic is generated by dpinger \cite{dpinger} and sends ICMP packets, whilst the second type is generated by hping3 \cite{hping3} and generates UDP/TCP packets. 
 %The probe traffic for a class $c$ enables our traffic monitoring tool to compute latency and loss values for all the traffic that pass through the class $c$. We also keep the DSCP value of probe traffic constant over time.
 %Generally, for each class $c$, dpinger sends echo requests (ICMP packets) every 100 milliseconds and keeps an array of all the echo requests. When a report is generated, the array is iterated to examine each echo request in order to compute latency. For each echo request, if the reply has been received, the time difference between the request and reply is computed (regarded as latency). If the response has not been received, the time since the request was sent is compared to the loss interval (400 ms). The request is then considered as loss if the value is more than the loss interval. However, if the missing reply is received later, its latency will be computed and it will no longer be marked as loss \cite{dpinger}. Besides latency and loss, dpinger also reports the jitter of the packets. 
 %On the other hand, hping3 is the advanced version of the ping program and can send ICMP, UDP and TCP packets. As we have used dpinger for ICMP packets, we use hping3 to send UDP/TCP packets. Hping3 measures the round-trip time (latency) of the packets sent to the destination and echoed back to the host. The statistical report of hping3 consists of packet loss, minimum, maximum and average of the round-trip times \cite{hping3}.

 %\textbf{sh: anything about the protocols of probe and test traffics?}
 %The main differentiating factor between a synthetic traffic and a probe traffic is that the synthetic traffic is  generated to consume a large bandwidth to stress the traffic shaping mechanism, while the bandwidth of the probe traffic is typically small and determined by the internals of the traffic monitoring tools. More precisely, the requested bandwidth of a probe traffic is negligible $\simeq 70$ bytes per second while the requested bandwidth of a synthetic traffic is large and close to the total bandwidth of its corresponding simulation scenario (e.g. 400 Mbps). Moreover, the protocol used for synthetic traffic is either UDP or TCP whereas the protocol of probe traffic can be any of the three mentioned protocols.
 
 






\\
%$ \mathit{MOS} = 1 + (0.035) \times \mathit{R\text{-}factor} + 0.000007 \times \mathit{R\text{-}factor} \times (\mathit{R\text{-}factor} - 60) \times (100 - \mathit{R\text{-}factor}) $






%\textbf{sh: moss is computed based on the three above. Can we describe here how moss is computed and why?}


%In addition, for each synthetic scenario $\mathit{tr}$, traffic shaping system computes the actual allocated bandwidth to $\mathit{tr}$ as an output, denoted by $\mathit{tr.actual$-$bw}$. For each traffic, we have $\mathit{tr.actual$-$bw} \leq \mathit{tr.req$-$bw}$. In addition, let $\mathit{tr}_1, \ldots, \mathit{tr}_m$ be synthetic traffics generated for the simulation scenario $\mathit{sc}$. We have $\sum_{1\leq l \leq m}\mathit{tr_l.actual$-$bw} \leq \mathit{total$-$bw}(sc)$. 

%\textbf{We need to index the actual bw by the simulation time step.}


%four metrics: latency, jitter, packet loss and MOS. Therefore, for a single test input $(\mathit{tr}_1, \ldots, \mathit{tr}_n)$ we have n $\times$ 4 outputs. 
%As a result, we need an aggregated and systematic metric for each test input to assess its quality and to be able to determine if the test input is close to the boundary behaviour of the system.
%We define a fitness function based on MOS values of classes. Such function should ideally have these behaviours: (1) Monotonicity: non-decreasing with respect to the order defined on the test inputs, (2) Have thresholds for boundary behaviours and can be interpreted by domain expert,  (3) Be quantitative (continuous)
%As MOS is derived based on latency, jitter and packet loss it compresses the effects of the other metrics. Hence, we use this metric for calculating the fitness. 
 %Next, we define the fitness function for test input i with n classes:



%\textbf{We can also define it in this way:}

%\begin{equation*}
%\displaystyle
%    F_i(MOS_1, \ldots, MOS_n) = \sum_{i = 1}^n \frac{1}{2}(sgn(i) + 1) + MOS_{\stackrel{max}{i = 1, \ldots, n}}\{
%    \frac{1}{2}|sgn(i) - 1|i
%    \}
%    \\
%\end{equation*}
%such that:
%\\
%$
%sgn(i) = 
%\begin{cases}
%    \frac{|MOS_i - mosthresh_i| + |mosthresh_i - MOS_i|}{2(MOS_i - mosthresh_i)} & MOS_i \neq mosthresh_i \\
%    1 & MOS_i = mosthresh_i
%\end{cases}
%$
%\\
%and
%$MOS_0 = 0$.
%\\

%The reason we don't go through the common part is that we can wind up with cases where there are no nodes remaining after reducing the path ($\mathit{length(P) = 0}$). As a result, we concentrate on the uncommon part, as we want to ensure that the path constrains at least some input variables. Second, the uncommon part is what distinguishes the two paths, and we want to know what input variable constraints result in changing from unacceptable to acceptable and vice versa. 
%For each predicate containing $tr_i$ in $C_u$, we calculate the \textit{final bound}. In particular the intersection of the upper or lower bounds of $tr_i$ is considered as the final upper or lower bound for $\mathit{tr_i}$ if multiple bounds are extracted:
%A path involves several conditions $\mathit{tr_i} \leq v$ or $\mathit{tr_i} > v$ where $v$ is considered as an upper or lower bound to $\mathit{tr_i}$ respectively.
%We extract all the conditions for $(\mathit{tr_1}, \ldots, \mathit{tr_n})$ from the non-robust paths. The intersection of the upper (lower) bounds is considered as the final upper (lower) bound for $\mathit{tr_i}$ if multiple bounds are extracted:
%\begin{itemize}
%    \item $\mathit{tr_i} \leq v_1 \land \mathit{tr_i} \leq v_2 \land v_1 \leq v_2 \to \mathit{tr_i} \leq v_1$
%    \item $\mathit{tr_i} > v_1 \land \mathit{tr_i} > v_2 \land v_1 \leq v_2 \to %\mathit{tr_i} > v_2$
%\end{itemize}
%\begin{itemize}
%    \item If $\mathit{tr_i} > v_1$ then the range is $[\mathit{max}(v_1 - \mathit{opt.Epsilon}, 0) , \mathit{min}(v_1 + \mathit{opt.Epsilon}, \mathit{bwTh}_i)]$
%    \item If $\mathit{tr_i} \leq v_1$ then the range is $[\mathit{max}(v_1 - \mathit{opt.Epsilon}, 0) , \mathit{min}(v_1 + \mathit{opt.Epsilon}, \mathit{bwTh}_i)]$
%\end{itemize}
%Specifically, assume that $[a, b]$ and $[c, d]$ are the ranges of $\mathit{tr_i}$ achieved from the previous iteration and $[a', b']$ and $[c', d']$ are the ranges obtained from the current iteration. If $(a' \leq a) \land (b \leq b')$ then $[a, b]$ $\subseteq$ $[a', b']$. Therefore, $[a, b]$ will be used for the next data generation. The same procedure applies to $[c, d]$ and $[c', d']$.
We sort the data points with respect to their weighted sum. In fact, for each data point we calculate 
$
\sum_{i = 1}^{n}w_i.\mathit{tr_i}
$
where $\mathit{w_i} = i$. 
%As a result, the fitness function mentioned in section~\ref{subsec:fitness} fulfills the required characteristics of a fitness function for our approach. 
To do so, assume that $R_1 = [x, y]$ and $R_2 = [h, g]$ are ranges of $\mathit{tr_i}$ in iteration i and $R'_1 = [a, b]$ and $R'_2 = [c, d]$ are ranges of $\mathit{tr_i}$ in iteration j where $i < j$. We have four cases in defining \textit{RangeSwing}:

\scalebox{0.45}{\begin{equation*}
    \mathit{RangeSwing(k, i, j) = } 
    \begin{cases}
        \frac{|x - a|}{max(|0 - x|,|x - \mathit{threshold_k}|)} & R_1 \neq \emptyset \land R_1' \neq \emptyset \land R_2 = \emptyset \land R_2' = \emptyset, \\
        \mathit{min}(\frac{|x - a|}{max(|0 - x|,|x - \mathit{threshold_k}|)},\frac{|h - a|}{max(|0 - h|,|h - \mathit{threshold_k}|)}) & R_1 \neq \emptyset \land R_2 \neq \emptyset \land R_1' \neq \emptyset \land R_2' = \emptyset, \\
        \mathit{min}(\frac{|x - a|}{max(|0 - x|,|x - \mathit{threshold_k}|)}, \frac{|x - c|}{max(|0 - x|,|x - \mathit{threshold_k}|)}) & R_1 \neq \emptyset \land R_1' \neq \emptyset \land R_2' \neq \emptyset \land R_2 = \emptyset, \\
        \frac{\mathit{min}(\frac{|x - a|}{max(|0 - x|,|x - \mathit{threshold_k}|)},\frac{|h - a|}{max(|0 - h|,|h - \mathit{threshold_k}|)}) + \mathit{min}(\frac{|x - c|}{max(|0 - x|,|x - \mathit{threshold_k}|)},\frac{|h - c|}{max(|0 - h|,|h - \mathit{threshold_k}|)})}{2} & R_1 \neq \emptyset \land R_2 \neq \emptyset \land R_1' \neq \emptyset \land R_2' \neq \emptyset
    \end{cases}
\end{equation*}}
%To minimize each path, let $\pi$ be the common prefix of $P_i$ and $P_k$. We denote the non-overlapping parts of $P_i$ and $P_k$ with $P_i\setminus\pi$ and $P_k\setminus\pi$, respectively. Let $C_i$ be the constraint obtained from $P_i\setminus\pi$, and $C_k$ be the constraint obtained from $P_k\setminus\pi$. A predicate is eliminated from $C_i$ (resp. $C_k$) if its corresponding node in $P_i$ (resp. $P_k$) split acceptable (resp. unacceptable) quality node from acceptable (resp. unacceptable) node.
%We intersect the predicates of $C_{tr_i}$ to have at most one predicate of form $tr_i > v$ (which we refer to as \textit{lower bound}) and at most one predicate of form $tr_i \leq v$ (which we refer to as \textit{upper bound}) for $tr_i$. Specifically, assume that $\mathit{tr_i} \leq v_1$ and $\mathit{tr_i} \leq v_2$ are two predicates in $C_{tr_i}$. If $v_1 \leq v_2$, then the upper bound of $tr_i$ is going to be $\mathit{tr_i} \leq v_1$. Similarly, if $\mathit{tr_i} > v_1$ and $\mathit{tr_i} > v_2$ are two predicates of $C_{tr_i}$ and $v_1 \leq v_2$, then $\mathit{tr_i} > v_2$ is the lower bound. We repeat this process until we have at most one upper bound and at most one lower bound for $tr_i$. In the example, the bounds extracted from $P_1$ and $P_2$ are $126 < \mathit{tr_1} \leq 126$, $79 < \mathit{tr_2} \leq 150$ and $\mathit{tr_3} \leq 6$.

%As mentioned in \textbf{RQ2}, our Baseline technique uses adaptive random testing to generate a set of test cases and executes those test cases on SOHOSim to generate test outputs. Finally, a regression tree is built using the generated test cases. Afterwards, the final ranges for each $tr_i$ is retrieved by passing the regression tree to Algorithm~\ref{alg:reduction}. The set of options and their values used for both algorithms (Baseline and ENRICH) are available at Table~\ref{tab:options}. We considered the average of robustness measures of our experiments as the value of $\mathit{opt.rbTh}$ in our experiments ($\mathit{opt.rbTh} = 3.6$).  The search budget is set to 15 iterations and within this budget, we first bootstrap each algorithm for 5 iterations (100 test cases) and afterwards, each algorithm generated 200 test cases. We set 15 iterations as our budget because ??


%for $m$ iterations and execute the new test cases on SOHOSim. If the output state has been changed within a specific number of steps (went from below $\mathit{opt.rbTh}$ to above it and vice versa), we consider $\mathit{tc_i}$ as a non-robust test case. are likely to be non-robust (i.e., their robustness measure may change from acceptable to unacceptable due to a small change in the input variables).


%we generate and execute a couple of test cases using the ranges generated by Baseline and ENRICH. The goal is to determine whether or not any of the generated test cases are likely to be non-robust (i.e., their robustness measure may change from acceptable to unacceptable due to a small change in the input variables). To do so, we make a small perturbation ($\delta$) in the input variables of each test input ($tc$) in at most $m$ consecutive iterations and determine whether or not, in $m$ iterations, the output state changes (i.e the quality of the system change from acceptable to unacceptable and vice versa). We start by calculating the robustness measures of the test inputs. If the robustness measure of $\mathit{tc_i}$ is below (resp. above) $\mathit{opt.rbTh}$, we deduct (resp. add) $\delta$ from (resp. to) each $tr_i$ for $m$ iterations and execute the new test cases on SOHOSim. If the output state has been changed within a specific number of steps (went from below $\mathit{opt.rbTh}$ to above it and vice versa), we consider $\mathit{tc_i}$ as a non-robust test case. The comparison metrics is $\mathit{NumberOfSteps}$ where we calculate in how many steps the test case changed state. The value of $\mathit{NumberOfSteps}$ is either in range $[1..m]$ or $\mathit{NULL}$ (the test case did not change state at all).


%Specifically, $\mathit{RangeSwing}$ computes the proportion of the gap between ranges $R$ and $R'$ over the

%If more than one range is obtained for $tr_i$ in an iteration, then $\mathit{RangeSwing}$ is the average of $\mathit{RangeSwing}$ for each pair of ranges (i.e. one range from previous iteration and one range from current iteration). The value of $\mathit{RangeSwing}$ is in range $[0..1]$ where $0$ indicates that the obtained ranges for $tr_i$ in two consecutive ranges were the same (ideal case), whereas $1$ indicates that the ranges were farther away.

%To answer this question, for each run of both algorithms, we generate 10 test cases. Next, we tweak each test case by $1\%$ of $\mathit{opt.TotalBandwidth}$ (i.e  we deduct or increment each $tr_i$ by $\delta$) for 5 consecutive steps. In other words, the maximum value subtracted/added from/to each $tr_i$ is $5.\delta$. The value of $\delta$ is chosen as a small number so that changes in the fitness can be tracked over a slower pace. As mentioned in section \ref{sec:experimentdesign}, The incrementation and deduction is decided based on the robustness measure of the test case. The number of steps that a test case takes to change state is stored in $\mathit{NumberOfSteps}$. 

%why do we need fitness
%We generate a lot of outputs for every single input vector. For example, see figure blah. We need an aggregated metric for each test input to assess its quality and to be able to determine if the test input is close to boundary behaviour of the system. Such function should ideally have these behaviours: (1) monotonic, (2) we can define threshold for boundary and can be interpreted by domain expert, (3) be quantitative (continuous). 

%The optimal $\mathit{ExtendEpsilon}$ is then chosen based on the highest values of precision and recall. To calculate the optimal number of runs to get optimal $\mathit{ExtendEpsilon}$, we randomly choose one run, two runs, three runs, ..., ten runs among the total number of runs that we have. Then, we label the test set again and calculate precision and recall. We repeat this process for $10$ times to account for randomness. The optimal number of runs is then chosen based on the highest value of precision and recall.   }
%arbitrary tests generated within the constrained ranges are non-robust. That is, we examine whether applying small perturbations to the inputs flips the robustness measure from acceptable to unacceptable or vice versa. We perform this analysis for both ENRICH and BASELINE.

%%%computed by ENRICH or BASELINE are non-robust (i.e., by applying small perturbations to their input elements, their robustness measure moves from acceptable to unacceptable or vice versa). 
%To do so, we generate and simulate a number of test inputs within the constrained ranges computed by ENRICH or BASELINE. 
%For each test input $\mathit{tc}$, if the calculated robustness measure is below (resp. above) $\mathit{rbTh}$, we deduct (resp. add) a small value $\delta$ from (resp. to) each input value in $\mathit{tc}$ and simulate the resulting test case (i.e., $\mathit{tc} \pm \delta$) to check if the robustness measure has moved from below $\mathit{rbTh}$ to above it, or vice versa. We keep modifying test inputs for a few steps. For each test input, we record whether the robustness measure crosses the threshold, and if so, after how many times of adding or subtracting $\delta$. In our experiments, we generate ten test inputs for each set of constrained ranges produced by either ENRICH or BASELINE. We note that since each simulation takes on average $5.4$min in our experimental setup, we limit the number of generated tests to ten.  We set $\delta = 1\%$ of the total bandwidth, and tweak test inputs up to four times. That is, the maximum perturbation applied to each input is $4\%$ of the total bandwidth. This is consistent with perturbations observed over a short time period (less than $1$sec) in network input flows in a SOHO setting. 


Figure~\ref{fig:5NRRP} shows the results of RQ1. Specifically, Figure~\ref{fig:5NRP} and Figure~\ref{fig:40NRP} show the results of first case study (i.e. Non robustness generation) and Figure~\ref{fig:5RP} and Figure~\ref{fig:40RP} show the results of second case study (i.e. robustness generation) for the lowest (i.e. $5$) and highest (i.e. $40$) values of $\varepsilon$. Based on Figure~\ref{fig:5NRP}, by setting $\varepsilon$ to $5$, on average, the highest value of non robustness precision and value of robustness recall are $0.86$ and $0.98$ respectively. On the other hand, when $\varepsilon = 40$, on average, the highest value of non robustness precision and robustness recall are $0.62$ and $0.54$ respectively. As a result, setting $\varepsilon$ to $5$ results in getting higher non robustness precision and robustness recall. Moreover, based on Figure~\ref{fig:5NRP}, the number of runs needed to get those values is three. Further, based on Figure~\ref{fig:5RP}, by setting $\varepsilon$ to $5$, on average, the highest value of robustness precision and non robustness recall are $0.81$ and $0.77$ and the highest value of robustness precision and non robustness recall when $\varepsilon = 40$, based on Figure~\ref{fig:40RP}, is $1$. Therefore, setting $\varepsilon$ to $40$ results in getting the highest robustness precision and non robustness recall (i.e. $1$) which can be achieved in five runs. \\
Furthermore, Figure~\ref{fig:threeorfive} demonstrates that how non robustness precision and robustness recall (resp. robustness precision and non robustness recall) change for ENRICH and BASELINE when running them for three (resp. five) times for different values of $\varepsilon$. Particularly, in Figure~\ref{fig:threeruns}, by increasing $\varepsilon$, overall the non robustness precision and robustness recall of ENRICH decrease. This is expected as by increasing $\varepsilon$, the ranges of ENRICH become wider and as a result, the number of tests predicted as Non Robust increases. Moreover, as discussed in Figure~\ref{fig:5NRP}, the highest value of non robustness precision and robustness recall for ENRICH is when $\varepsilon = 5$. At this $\varepsilon$, there is a significant difference between the non robustness precision and robustness recall of BASELINE and ENRICH. Further, in Figure~\ref{fig:fiveruns}, when $\varepsilon$ increases the robustness precision and non robustness recall of ENRICH increases. For instance, when $\varepsilon = 40\%$, the ranges of ENRICH are wide enough and can label the robustness class with $100\%$ precision and cover all of the non robust tests. Although, for $\varepsilon = 40\%$, BASELINE fully covers all the non robust classes, it fails to precisely label robust classes. The reason is that for $\varepsilon = 40\%$, the ranges of BASELINE become very wide and as a result, all the tests fall into the ranges of BASELINE and are predicted as Non robust.

We first calculate the standard precision and recall for Robust and Non Robust classes for the lowest (i.e. $5$) and highest (i.e. $40$) values of $\varepsilon$ for $20$ different combination of runs of ENRICH. 
Specifically, we have studied two possible case studies for our parameterized ranges: (1) Non Robustness generation, (2) Robustness generation. In the former case, in order to generate non robust tests from the ranges, we analyze the precision of non robustness class and recall of robustness class. In the latter case, we analyze the precision of robustness class and recall of non robustness class. In other words, the higher the precision of non robustness (resp. robustness) class, the more accurate the parameterized ranges are in classifying non robust (resp. robust) classes. Further, the higher the recall of robustness (resp. non robustness) class, the more capable the ranges are in covering robust (resp. non robust) classes.
We recalculate the ranges with respect to the lowest and highest values of $\varepsilon$ and analyze if the ranges of any of the runs covers any of the test inputs. In that case, that test input is predicted as Non Robust. Otherwise, it is predicted as Robust. We then analyze in how many runs the maximum precision and recall is achieved for both case studies. 

\begin{figure}
    \centering
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/25 RP-NRR.pdf}
        \caption{Robustness Precision and Non Robustness Recall of ENRICH for $\varepsilon = 25$.}
        \label{fig:25RP}
    \end{subfigure}
    
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/25 RP-NRR-base.pdf}
        \caption{Robustness Precision and Non Robustness Recall of BASELINE for $\varepsilon = 25$.}
        \label{fig:25RPbaseline}
    \end{subfigure}
    
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/30 RP-NRR.pdf}
        \caption{Robustness Precision and Non Robustness Recall of ENRICH for $\varepsilon = 30$.}
        \label{fig:30RP}
    \end{subfigure}
    
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/30 RP-NRR-base.pdf}
        \caption{Robustness Precision and Non Robustness Recall of BASELINE for $\varepsilon = 30$.}
        \label{fig:30RPbaseline}
    \end{subfigure}
    
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/35 RP-NRR.pdf}
        \caption{Robustness Precision and Non Robustness Recall of ENRICH for $\varepsilon = 35$.}
        \label{fig:35RP}
    \end{subfigure}
    
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/35 RP-NRR-base.pdf}
        \caption{Robustness Precision and Non Robustness Recall of BASELINE for $\varepsilon = 35$.}
        \label{fig:35RPbaseline}
    \end{subfigure}
    
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/40 RP-NRR.pdf}
        \caption{Robustness Precision and Non Robustness Recall of ENRICH for $\varepsilon = 40$.}
        \label{fig:40RP}
    \end{subfigure}
    
    \begin{subfigure}[]{\columnwidth}
        \includegraphics[width=\columnwidth]{figs/40 RP-NRR-base.pdf}
        \caption{Robustness Precision and Non Robustness Recall of ENRICH for $\varepsilon = 40$.}
        \label{fig:40RPbaseline}
    \end{subfigure}
    \caption{Comparison of Robustness Precision and Non Robustness Recall of ENRICH and BASELINE for  $\varepsilon$ between $25$ and $40$.}\label{fig:25to40}
    
\end{figure}

\begin{figure}
   \centering
\begin{tabular}{p{4cm}p{4cm}}
\multicolumn{2}{c}{Robustness Precision and Non Robustness Recall}\\
\multicolumn{2}{c}{}\\
\multicolumn{1}{c}{ENRICH} & \multicolumn{1}{c}{BASELINE} \\
\includegraphics[width=0.5\columnwidth]{figs/25 RP-NRR.pdf}&
\includegraphics[width=0.5\columnwidth]{figs/25 RP-NRR-base.pdf}\\
\multicolumn{1}{c}{(a) $\varepsilon = 25$} &
\multicolumn{1}{c}{(b) $\varepsilon = 25$} \\
\includegraphics[width=0.5\columnwidth]{figs/30 RP-NRR.pdf}&
\includegraphics[width=0.5\columnwidth]{figs/30 RP-NRR-base.pdf}\\
\multicolumn{1}{c}{(c) $\varepsilon = 30$} &
\multicolumn{1}{c}{(d) $\varepsilon = 30$} \\
\includegraphics[width=0.5\columnwidth]{figs/35 RP-NRR.pdf}&
\includegraphics[width=0.5\columnwidth]{figs/35 RP-NRR-base.pdf}\\
\multicolumn{1}{c}{(e) $\varepsilon = 35$} &
\multicolumn{1}{c}{(f) $\varepsilon = 35$} \\
\includegraphics[width=0.5\columnwidth]{figs/40 RP-NRR.pdf}&
\includegraphics[width=0.5\columnwidth]{figs/40 RP-NRR-base.pdf}\\
\multicolumn{1}{c}{(g) $\varepsilon = 40$} &
\multicolumn{1}{c}{(h) $\varepsilon = 40$} \\
\end{tabular}
   \caption{Comparison of Robustness Precision and Non Robustness Recall of ENRICH and BASELINE for  $\varepsilon$ between $25$ and $40$ over different combination of runs.}\label{fig:25to40}
\end{figure}
